Random Feature Stein Discrepancies

Computable Stein discrepancies have been deployed for a variety of applications, ranging from sampler selection in posterior inference to approximate Bayesian inference to goodness-of-fit testing. Existing convergence-determining Stein discrepancies admit strong theoretical guarantees but suffer from a computational cost that grows quadratically in the sample size. While linear-time Stein discrepancies have been proposed for goodness-of-fit testing, they exhibit avoidable degradations in testing power -- even when power is explicitly optimized. To address these shortcomings, we introduce feature Stein discrepancies ($\Phi$SDs), a new family of quality measures that can be cheaply approximated using importance sampling. We show how to construct $\Phi$SDs that provably determine the convergence of a sample to its target and develop high-accuracy approximations -- random $\Phi$SDs (R$\Phi$SDs) -- which are computable in near-linear time. In our experiments with sampler selection for approximate posterior inference and goodness-of-fit testing, R$\Phi$SDs perform as well or better than quadratic-time KSDs while being orders of magnitude faster to compute.

==> error_bound_examples.tex <==
%
%
\subsection{Explicit examples} \label{sec:examples}
The results of \cref{sec:error-bounds,sec:reference-mmd} allow us to develop explicit convergence-determining {\FGMMD}s with $(C,\gamma)$ second moments for any $\gamma > 0$.
We give two examples, corresponding to the {\FGMMD}s used in our experiments.
Without loss of generality, as in \cref{thm:FGMMD-c-alpha-second-moment}, we assume that $\mean{\targetdist} = 0$.
In each example, we first fix target smoothness and tail parameters $\overline{\lambda}$ and $\xi$; these define a range of achievable importance sample growth rates $\gamma$ via \cref{thm:FGMMD-c-alpha-second-moment}.  
We next introduce a convergence-determining reference KSD with Stein kernel \cref{eqn:stein-kernel} 
written in the canonical form \cref{eqn:sqrt-decomp}; together with a choice of $r$, the decomposition into $\sqrtkvec$ and $\rho$ fully determines the associated GMMD.
Finally, we prove both that the assumptions of \cref{thm:FGMMD-c-alpha-second-moment} are met when all the $\gj$ are chosen equal and
$\nu\propto\gj[1]^{\xi r}$, guaranteeing $(C,\gamma)$ second moments,
and that $\rho  = \FT{\Phi}_1/\wideFT{\gj[1]}^2$ has bounded $\Lp{t}$ norm, guaranteeing that the GMMD upper bounds the KSD by \cref{eqn:mmd-ipm-bound}.


\bexa[$\Lp{2}$ tilted sech {\FGMMD}] \label{exa:tilted-sech}

Take $\overline{\lambda} = 1$, fix any $\xi \in (0,1)$, and choose an inverse scale parameter $a > 0$.
Recall that the hyperbolic secant (sech) function is given by $\sech(u) = \frac{2}{e^{u} + e^{-u}}$.
For $x \in \reals^D$, define the sech kernel
$
\sechK{a}(x) %
\defined \prod_{d=1}^D \sech\left(\sqrt{\frac{\pi}{2}}ax_d\right).
$

Consider a reference KSD with tilted sech base kernel $\kernel(x, y) = \kernelMultFun(x - \mean{\approxdist[N]})\sechK{a}(x - y)\kernelMultFun(y - \mean{\approxdist[N]})$,
where $\kernelMultFun$ is any positive, differentiable function. 
%
%
%
%
%
%
The induced Stein kernel $k_0$ from \cref{eqn:stein-kernel} has canonical form \cref{eqn:sqrt-decomp} with $J=D$
and, for each $j\in[J]$, $\gj = \sechK{2a}$,  $\sqrtk[j](x, \omega) = \FTop(\mcT_{j,x}\kernelMultFun(x  - \mean{\approxdist[N]})\gj(x - \cdot))(\omega)$, and 
 $\rho = (\FTsechK{2a})^{2}/\wideFT{\gj}^2 = 1$.
As shown in \cref{sec:tilted-sech-fgmmd-properties-proof}, with the choice of $r = 2$ and $\nu(z) \propto \sechK{2a}(z  - \mean{\approxdist[N]})^{2\xi}$
or  $\nu(z) \propto \approxdist[N](\sechK{2a}(z  - \cdot)^{2\xi})$, 
the resulting $\Lp{2}$ IMQ {\FGMMD} meets all of our relative error criteria.
\notate{Mention that it's easy to sample from this distribution.}

\notate{Make propositions}
\bnthm[$\Lp{2}$ tilted sech {\FGMMD} properties] \label{thm:tilted-sech-fgmmd-properties}
Under the settings of \cref{exa:tilted-sech}, let $\mcQ^{\mathrm{sech}}(C)$ denote the family of distributions for which %
%
\[
\approxdist[N]((1 + \onenorm{\cdot})\kernelMultFun(\cdot  - \mean{\approxdist[N]}) e^{\sqrt{\frac{\pi}{2}}a \onenorm{\cdot - \mean{\approxdist[N]}}}) &\le C. %
%
\]
Assume that $\targetdist \in \pset$ and that for some constants $C_{1}, C_{2} \ge 0$,
\[
\onenorm{\grad \log \kernelMultFun(x)} &\le C_{1} + C_{2} \onenorm{x}. \label{eq:norm-grad-A-bound}
\]
Then, in the notation of \cref{thm:FGMMD-c-alpha-second-moment},
for any $b > 0$, $(\sqrtkvec,r,\isdist)$ yields $(C_{\alpha}, \gamma_{\alpha})$ 
second moments for $\targetdist$ and $\mcQ^{\mathrm{sech}}(C)$.
Moreover, $\MMD_{\kernel_0}^2 = \GMMD^{2}_{\sqrtkvec,2}.$
\enthm
\,
\eexa
%
\bexa[$\Lp{r}$ IMQ {\FGMMD}] \label{exa:imq}
Fix any $\overline{\lambda} \in (1/2,1)$, $\underline{\xi} \in (0,1/2)$, and $\xi \in (\underline{\xi},1)$.
Consider a reference KSD with IMQ base kernel 
$k(x,y) = \IMQ{c}{\beta}(x-y)$ with $c > 0$ and $\beta \in [-D/2,0)$.
For $c' = \overline{\lambda} c/2$ and any $\beta' \in [-D/(2\underline{\xi}), -\beta/(2\underline{\xi})-D/(2\underline{\xi}))$, 
the induced Stein kernel $k_0$ from \cref{eqn:stein-kernel} has canonical form \cref{eqn:sqrt-decomp} with $J=D$, and,
for each $j\in[J]$, $\gj = \IMQ{c'}{\beta'}$, $\sqrtk[j](x, \omega) = \FTop(\mcT_{j,x}\gj(x - \cdot))(\omega)$, and 
 $\rho = \FTIMQ{c}{\beta}/\wideFT{\gj}^2$.
As shown in \cref{sec:imq-fgmmd-properties-proof}, with the choice of 
$r=-D/(2\beta'\underline{\xi})$ and $\nu(z) \propto \IMQ{c'}{\beta'}(z - \mean{\approxdist[N]})^{\xi r}$
or $\nu(z) \propto \approxdist[N](\IMQ{c'}{\beta'}(z - \cdot)^{\xi r})$, 
the resulting $\Lp{r}$ IMQ {\FGMMD} meets all of our relative error criteria.
%
\bnthm[$\Lp{r}$ IMQ {\FGMMD} properties] \label{thm:imq-fgmmd-properties}
Under the settings of \cref{exa:imq}, let $\mcQ^{\mathrm{IMQ}}(C) $ denote the family of distributions 
for which %
\[
\approxdist[N](\twonorm{\cdot}\twonorm{\cdot - \mean{\approxdist[N]}}^{-2\beta'}) &\le C. %
%
\label{eq:IMQ-Q-moment-bound}
\]
Assume that $\targetdist \in \pset$.
Then, in the notation of \cref{thm:FGMMD-c-alpha-second-moment}, for $b = 0$,
$(\sqrtkvec,r,\isdist)$ yields $(C_{\alpha}, \gamma_{\alpha})$ second moments for $\targetdist$ and $\mcQ^{\mathrm{IMQ}}(C)$.
Moreover, there exists a constant $C' > 0$ such that for any $\approxdist[N]$
\[
\MMD_{\kernel_0}^2(\approxdist[N],\targetdist) \le C'\GMMD^{2}_{\sqrtkvec,r}(\approxdist[N],\targetdist).
\]
\enthm
A particularly simple setting is given by $\beta' = -D/(2\underline{\xi})$ which yields $r = 1$.
\eexa


==> error_bounds.tex <==
%

%
\subsection{Selecting an importance sampling function $\nu$} %
\label{sec:error-bounds}

We next turn to developing high-probability relative error bounds for {\FGMMD}s with sub-quadratic sample complexity.
Our strategy is to show that the second moment of each {\FGMMD} feature, $w_{j}(Z, \inducingoperator[N]) \defined |(\invFTop\inducingoperator[N] \sqrtk[j])(Z)|^r/\isdist(Z)$, is bounded by a power of its mean:
\bnumdefn[$(C,\gamma)$ second moments]
\label{defn:second-moment-property}
Fix a target distribution $\targetdist$ and a family of distributions $\mcQ$. 
For $Z\dist \nu$ and $j \in [J]$, let $Y_{j} \defined w_{j}(Z, \inducingoperator[N])$. %
If for some $C > 0$ and $\gamma \in [0,2]$, for all $\approxdist[N] \in \mcQ$, 
\[
%
\EE[Y_j^2] \le C \EE[Y_j]^{2-\gamma},
\] 
%
then we say $(\sqrtkvec,r,\isdist)$ yields
\emph{$(C,\gamma)$ second moments for $\targetdist$ and $\mcQ$}.
\enumdefn
%
The next proposition, proved in \cref{sec:estimated-ksd-lb-guarantee-proof}, demonstrates the value of this second moment property.
%
\bnprop \label{prop:estimated-mmd-lb-guarantee}
%
If $(\sqrtkvec,r,\isdist)$ yields $(C,\gamma)$ second moments for $P$ and $\mcQ$
and $M \ge 2C\EE[Y_j]^{-\gamma}\log(J/\delta)/\eps^2$ for all $j \in [J]$, then,
for any $\approxdist[N] \in \mcQ$, with probability at least $1-\delta$, 
\baligns
\FGMMD_{\sqrtkvec,r,\isdist,M}
	&\ge (1-\eps)^{1/r}\GMMD_{\sqrtkvec, r}.
\ealigns
\enprop
When $\norm{\rho}_{\Lp{s}} < \infty$ and $\MMD_{k_0}^2(Q_N,P) = \Omega(N^{-1})$, \cref{prop:estimated-ksd-lb-guarantee} and the MMD-GMMD inequality \cref{eqn:mmd-ipm-bound} imply that a $(C,\gamma)$ {\FGMMD} dominates its reference MMD with high probability whenever the importance sample size $M = \Omega(N^{\gamma\;\!r/2})$.
Note that  $\MMD_{k_0}^2(Q_N,P) = \Omega_P(N^{-1})$ whenever the sample points $x_1, \dots, x_N$ are drawn i.i.d.\ from a distribution $Q$, since the scaled V-statistic $N \MMD_{k_0}^2(Q_N,P)$ diverges when $Q\neq P$ and converges in distribution to a non-zero limit when $Q=P$ \citep[Thm. 32]{sejdinovic2013equivalence}.
Moreover, working in a hypothesis testing framework of shrinking alternatives, \citet[Thm. 13]{Gretton:2012} showed that $\MMD_{k_0}^2(Q,P) = \Theta(N^{-1})$ was the smallest local departure distinguishable by an asymptotic MMD test.
\notate{Highlight $r$ benefits}
\notate{ Discuss the following here or in the "special cases" section: 
Popular approaches approximate the MMD in $\Theta(NM)$ time using a finite feature expansion of size $M$ based on random Fourier features~\citep{Rahimi:2007,zhao2015fastmmd,sutherland2015error,Sriperumbudur:2015,Honorio:2017},
other types of randomly sampled features~\citep{Dai:2014,Chwialkowski:2015,Bach:2017,Briol:2017,Jitkrittum:2017}, or the \Nystrom method~\citep{WilliamsSe00,Yang:2012,Musco:2017}. 
However, existing analyses only guarantee $O_P(M^{-1/2})$-precision estimates of the reference MMD
and require $\Theta(N^2)$ time to achieve the typical $\Theta(N^{-1/2})$ precision of the reference MMD.
%
}

We next turn to establishing practical sufficient conditions that imply $(C,\gamma)$ second moments.
Notably, any improvements on these second moment bounds translate directly into improved sample complexity bounds for {\FGMMD}s.

%
Our first result, proved in \cref{sec:FGMMD-c-1-second-moment-proof}, 


\notate{Don't do any rewriting of the GKSD; instead, give all conditions (as simply as possible) in terms of the GKSD representation we initially provide.}

\notate{Some of the refined assumptions discussed at our last meeting:
\benumerate
\item $\hat{\psi}^{1/2 - \lambda /2} \in L^2$
\item $\omega_j^2 \hat{\psi}^{1/2} \in L^1$
\item Integrability assumption for Q
\item Growth assumption for $\psi$ and/or its derivative
\eenumerate
}
A more refined analysis provides sufficient conditions 
for $(C,\gamma)$ second moments for any $\gamma > 0$.
The key condition is a structural assumption about $\sqrtk[j]$:
\begin{assumption} \label{asm:kj-form}
For all $j \in [J]$, $\sqrtk[j](x, \omega) = \FTop(\linop{j}{x}\gj(x - \cdot))(\omega)$, 
where $\linop{j}{x}$ is a linear operator and $\gj$ is a symmetric function. 
\end{assumption}
Let 
\[ 
\kj[j](x, y) \defined \int \sqrtk[j](x,\omega) \overline{\sqrtk[j](y,\omega)} \rho(\omega) \domega,
\]
so if $\kernel_{0}$ is of the form \cref{eqn:sqrt-decomp}, $\kernel_{0} = \sum_{j=1}^{J} \kj[j]$. 
As shown in \cref{sec:kj-rewrite-proof}, \cref{asm:kj-form} leads to a convenient rewriting of the kernel components $\kj[j]$
in terms of the linear operators acting on a stationary kernel:
\bnprop  \label{prop:kj-rewrite}
Under \cref{asm:kj-form}, 
\(
\kj[j](x,y) = \linop{j}{x}\linop{j}{y}\statKernj(x - y),
\)
where $\FTstatKernj \defined \wideFT{\gj}^{2} \rho$.
Hence 
\(
(\inducingoperator[N] \times \inducingoperator[N]) \kernel_{0}
%
= \textsum_{j=1}^{J}\norm{\textint\linop{j}{x}\statKernj(x - \cdot)\inducingoperator[N](\dee x)}_{\statKernj}^{2}.
\)
\enprop


We also require two additional conditions, which concern how $\gj$ relates to $\FTstatKernj$ 
and $\isdist$ relates to $\gj$. 
Specifically, $\gj$ must be sufficiently smooth:
\begin{assumption} \label{asm:gj-in-phij-alpha}
There exists a \emph{smoothness parameter} $\overline{\lambda} \in (1/2, 1]$ such that if $\lambda \in (1/2, \overline{\lambda})$, then $\wideFT{\gj}/\FTstatKernj^{\lambda/2} \in \Lp{2}$.
%
\end{assumption}
Requiring that $\wideFT{\gj}/\FTstatKernj^{\lambda/2} \in \Lp{2}$ is equivalent to requiring that $\gj$ belong to the
reproducing kernel Hilbert space $\kset_{\lambda}$ induced by the kernel $\invFTop(\FTstatKernj^{\lambda})$. 
The smoothness of the functions in $\kset_{\lambda}$ increases as $\lambda$ increases.
Hence $\overline{\lambda}$ quantifies the smoothness of $\gj$ relative to $\statKernj$. 
 
For a distribution $\genericdist$, let $\mean{\genericdist} \defined \EE_{X \dist \genericdist}[X]$ denote the mean of $\genericdist$ (if it exists) and $\infty$ otherwise. 
The importance distribution $\isdist$ must also be heavy-tailed relative to $\gj$:
\begin{assumption} \label{asm:inverse-nu-bound}
$\mean{\approxdist[N]} < \infty$ and 
there exists a \emph{tail parameter} $\xi \in (0,1)$ 
such that for $j \in [J]$, for some $C_{\isdist,j} > 0$, and for all $z \in \reals^{d}$,
$\isdist^{-1}(z) \le C_{\isdist,j}\gj^{-\xi r}(z - \mean{\approxdist[N]})$.
\end{assumption}
\cref{asm:inverse-nu-bound} results in over-dispersed features relative to $\gj$, which
ensures that regions of mismatch between $\targetdist$ and $\approxdist[N]$ are picked up
by the {\FGMMD}. 
In addition to \cref{asm:kj-form,asm:gj-in-phij-alpha,asm:inverse-nu-bound},
our result (proved in \cref{sec:second-moment-bounds}) relies on several other regularity conditions.
The statement of these conditions is deferred to \cref{sec:second-moment-bounds}.

%
\bnthm \label{thm:FGMMD-c-alpha-second-moment}
%
Assume that $\targetdist \in \pset$, without loss of generality that $\mean{\targetdist} = 0$,
and that \cref{asm:kj-form,asm:gj-in-phij-alpha,asm:hat-phi-integrability,asm:product-function-bound,asm:inverse-nu-bound,asm:f-decreasing} hold.
%
%
Let $\mcQ(C_{\isdist,j},b,C_{B,j},C_{\mcO,j})$  denote the family of distributions  for which %
\cref{asm:inverse-nu-bound,asm:Delta-Bj-bound,asm:FT-linop-bound} hold for some uniform choice of the constants $C_{\isdist,j}, b, C_{B,j}$, and $C_{\mcO,j}$.
For $\alpha > 2(1 - \overline{\lambda})$, let $\gamma_{\alpha} \defined \alpha + (2 - \alpha)\xi/(2-b-\xi)$.
Then for a constant $C_{\alpha} > 0$, $(\sqrtkvec,r,\isdist)$ yields $(C_{\alpha}, \gamma_{\alpha})$ second moments 
for $\targetdist$ and $\mcQ(b,C_{B,j},C_{\mcO,j})$.
\enthm

\cref{thm:FGMMD-c-alpha-second-moment} suggests a strategy for improving the importance 
sample growth rate $\gamma$ of an {\FGMMD}: increase the smoothness $\overline{\lambda}$ of $\gj$ and 
decrease the tail parameter $\xi$ to increase the over-dispersion of $\nu$ relative to $\gj$.


%
\input{error_bound_examples.tex}

==> reference_mmd.tex <==
%

%
\subsection{Selecting a feature function $\feat$} 
\label{sec:reference-mmd}
\notate{Our next result both upper and lower bounds the GKSD by a more familiar KSD, showing that the GKSD determines weak convergence whenever the KSD does: TODO: write this result.
}

Few KSDs are known to determine weak convergence on $\reals^d$. 
A notable exception is the KSD with inverse multiquadric (IMQ) base kernel
$k(x,y) = \IMQ{c}{\beta}(x-y) \defined (c^2 + \twonorm{x-y}^2)^\beta$ for $c>0$ and $\beta \in (-1,0)$.
\citet[Thm. 8]{Gorham:2017} proved that these IMQ KSDs 
determine weak convergence on $\reals^d$ whenever $P\in\pset$, the set of distantly dissipative distributions with Lipschitz $\grad \log p$.
We say $P$ satisfies \emph{distant dissipativity}~\cite{Eberle:2015,Gorham:2016b} if $\kappa_0 \defined \lim\inf_{r\to\infty} \kappa(r) > 0$ for
$$
\kappa(r) = \inf \{ -2 \textfrac{\inner{\grad\log p(x)-\grad\log p(y)}{x-y}}{\twonorm{x-y}^2} : \twonorm{x-y} = r \} .
$$
An IMQ KSD will serve as the convergence-determining reference MMD for our $L^r$ IMQ {\FGMMD}s developed in \cref{exa:imq}.

Our next result, proved in \cref{sec:tilted-weak-convergence-proof}, shows that tilted base kernels of the form $A(x) \Phi(x-y) A(y)$ also determine convergence to $\pset$.
%
\begin{nthm}[Tilted KSDs determine convergence]
\notate{TODO: check that we can replace $A(x)$ with $A(x - \mean{\approxdist})$ here}
Suppose that $P\in\pset$ and that $k(x,y) = A(x)\Phi(x-y)A(y)$ for 
$\Phi \in C^2$ with $F(u) = \sup_{\omega \in\reals^d} e^{-\twonorm{\omega}^2/(2u^2)}/\hat{\Phi}(\omega)$ finite for all $u > 0$
and
$A \in C^1$ with $A > 0$, $1/A \in \Lp{2}$, and bounded-Lipschitz $\grad \log A$. 
Then, for any sequence of probability measures $(\mu_n)_{n=1}^\infty$, $\mu_n \convD P$ whenever $\KSD_k(\mu_n,P) \to 0$.
\end{nthm}
\notate{Did we define this KSD notation?}
\cref{thm:tilted-weak-convergence} motivates the new convergence-determining tilted hyperbolic secant kernels introduced in \cref{exa:tilted-sech}.


\notate{End with assumptions on feature function motivated by the results above $\feat(x,z) = A(x) \psi(\norm{x-z})$}


For a distribution $\genericdist$, let $\mean{\genericdist} \defined \EE_{X \dist \genericdist}[X]$ denote the mean of 
$\genericdist$ (if it exists) and $\infty$ otherwise. 
We will assume that $\mean{\approxdist} < \infty$, which always holds when $\approxdist$ is a discrete distribution with finite support.





\begin{assumption} 
\cref{asm:feature-form} holds and for any $\xi \in (0,1/2)$,
and any $\approxdist$ with $\mean{\approxdist} < \infty$, 
$Q(\statfeat(z - \cdot)^{2\xi}) \ge L(\approxdist) \statfeat(z - \mean{\approxdist})^{2\xi}$, 
where $L(\approxdist) \ge 0$. 
\end{assumption}

==> shortcuts.tex <==
\makeatletter
\def\widebreve#1{\mathop{\vbox{\m@th\ialign{##\crcr\noalign{\kern\p@}%
  \brevefill\crcr\noalign{\kern0.1\p@\nointerlineskip}%
  $\hfil\displaystyle{#1}\hfil$\crcr}}}\limits}

\def\brevefill{$\m@th \setbox\z@\hbox{}%
 \hfill\scalebox{0.7}{\rotatebox[origin=c]{90}{(}} \kern4pt $}
\makeatletter

% TODO:
% - decide on whether to use bold notation for vectors 
% - settle on consistent operator notation (e.g., use hats?)
% - settle on RKHS, unit ball, and RKHS norm notations
% - settle on consistent derivative notations 
%
% Conflicting notation
% nu = matern order OR sqrt distribution
% a = used to define order of Matern kernel OR generic scalar
% b = score function OR generic scalar

% (asymptotic) equivalance 
\newcommand{\asympequiv}{\sim} % asymptotically equivalent
\newcommand{\asympequivconst}{\mathbin{\dot{\sim}}} % asymptotically equivalent up to a positive constant
\newcommand{\equivconst}{\doteq} % equivalent up to a const: a equivconst b iff 

% making fractions easier
\newcommand{\fracexp}[3]{\left(\frac{#1}{#2}\right)^{#3}}
\newcommand{\gammafrac}[2]{\frac{\Gamma(#1)}{\Gamma(#2)}}

% hyperbolic functions
\newcommand{\sech}{\operatorname{sech}}

% binary operators
\newcommand{\minop}{\mathbin{\wedge}}
\newcommand{\maxop}{\mathbin{\vee}}
\newcommand{\convolve}{\mathbin{*}}
\newcommand{\vol}{\operatorname{vol}}

% measures
\newcommand{\Lebesgue}{\lambda}
\newcommand{\sqrtdist}{\nu}
\newcommand{\isdist}{\nu}
\newcommand{\genericdist}{\mu}
\newcommand{\sourcedist}{\mu}
\newcommand{\approxdist}[1][]{Q_{N}}
\newcommand{\approxdistN}{Q_{N}}
\newcommand{\approxdensity}[1][]{q_{}}
\newcommand{\targetdist}{P}
\newcommand{\targetdensity}{p}
\newcommand{\mean}[1]{m(#1)}
\newcommand{\approxmean}{m_{N}}
\newcommand{\targetmean}{m_{\targetdist}}
\newcommand{\distvar}[1]{\sigma(#1)^{2}}
\newcommand{\diststdev}[1]{\sigma(#1)}


% Lp norms
\newcommand{\Lp}[1]{L^{#1}}
\newcommand{\Lpnorm}[2]{\norm{#2}_{\Lp{#1}}}
\newcommand{\staticLpnorm}[2]{\staticnorm{#2}_{\Lp{#1}}}
\newcommand{\Lpinner}[3]{\inner{#2}{#3}_{\Lp{#1}}}
\newcommand{\Lparg}[2]{L^{#1}(#2)}
\newcommand{\Lpnormarg}[3]{\norm{#3}_{\Lparg{#1}{#2}}}
\newcommand{\staticLpnormarg}[3]{\staticnorm{#3}_{\Lparg{#1}{#2}}}
\newcommand{\Lpinnerarg}[4]{\inner{#3}{#4}_{\Lparg{#1}{#2}}}

\newcommand{\Lnu}{\Lparg{2}{\sqrtdist}}

% Fourier transforms and distributions
\newcommand{\FT}[1]{\hat{#1}} % Fourier transform
\newcommand{\invFT}[1]{\breve{#1}} % inverse Fourier transform
\newcommand{\wideFT}[1]{\widehat{#1}} % Fourier transform
\newcommand{\wideinvFT}[1]{\widebreve{#1}} % inverse Fourier transform
\newcommand{\FTop}[0]{\mathscr{F}} % Fourier transform
\newcommand{\invFTop}[0]{\FTop^{-1}} % inverse Fourier transform
\newcommand{\FTdop}[0]{\FTop_d} % d-dimesional scalar Fourier transform
\newcommand{\invFTdop}[0]{\invFTop_d} % d-dimensional scalar inverse Fourier transform
\newcommand{\Schwartz}[0]{\mathcal{S}} % \Schwartz space
\newcommand{\tempered}[0]{\mathcal{S}'} % Space of tempered distributions
\newcommand{\dists}[0]{\mathcal{D}'} % Space of distributions
\newcommand{\jbracket}[1]{\langle{#1}\rangle} % Japanese bracket < x > := (1 + |x|^{2})^{1/2}
\newcommand{\FTpow}[2]{#1^{(#2)}} % f^(s) := FT^-1((FT f)^s)
\newcommand{\FTsqrt}[1]{\FTpow{#1}{1/2}}

% Kernels and related things
\newcommand{\kernel}{k}
\newcommand{\sqrtk}[1][]{\kernel^{1/2}_{#1}} % square root kernel
\newcommand{\kj}[1][j]{\kernel_{#1}} 
\newcommand{\sqrtkvec}[0]{\boldsymbol\kernel^{1/2}} % square root kernel
\newcommand{\statKern}{\Phi} % stationary kernel
\newcommand{\statKernScalar}{\phi} % stationary kernel
\newcommand{\kernelMultFun}{A} % for defining the kernel k_A(x,y) = A(x)Phi(x - y)A(y)
\newcommand{\linop}[2]{\mcO_{#1,#2}}
\newcommand{\gj}[1][j]{f_{#1}}
\newcommand{\gjbound}[1][j]{\overline{\gj[#1]}}
\newcommand{\grhoj}[1][j]{h_{#1}}
\newcommand{\FTgrhoj}[1][j]{\FT{h}_{#1}}
\newcommand{\statKernj}[1][j]{\statKern_{#1}}
\newcommand{\FTstatKernj}[1][j]{\FT{\statKern}_{#1}}
\newcommand{\wj}[1][j]{w_{#1}}
\newcommand{\fa}{f_{1}}
\newcommand{\fb}{f_{2}}
\newcommand{\fc}{f_{3}}
\newcommand{\find}{f_{i}}
\newcommand{\Ua}{U_{1}}
\newcommand{\Ub}{U_{2}}
\newcommand{\Uind}{U_{i}}

\newcommand{\BesselK}[1]{K_{#1}}  % modified Bessel function of the second kind
\newcommand{\MaternK}[2]{\Phi_{#1,#2}}  % (normalized) Matern kernel
\newcommand{\MaternKScalar}[2]{\phi_{#1,#2}}  % (normalized) Matern kernel, scalar arg
\newcommand{\sechK}[1]{\Psi_{#1}^{\mathrm{sech}}}  % (normalized) sech kernel
\newcommand{\FTsechK}[1]{\FT{\Psi}_{#1}^{\mathrm{sech}}}  % (normalized) sech kernel
\newcommand{\IMQ}[2]{\Psi^{\mathrm{IMQ}}_{#1,#2}} % inverse multi-quadric kernel
\newcommand{\FTIMQ}[2]{\FT{\Psi}^{\mathrm{IMQ}}_{#1,#2}} % inverse multi-quadric kernel
\newcommand{\IMQScalar}[2]{\psi_{#1,#2}} % inverse multi-quadric kernel, scalar arg
\newcommand{\Gaussian}[1]{\Lambda_{#1}}  % Gaussian kernel
\newcommand{\GaussianScalar}[1]{\lambda_{#1}}  % Gaussian kernel

% Stein and MMD stuff
\newcommand{\inducingoperator}[1][]{\Delta_{#1}} % stands in for MMD- or Stein-inducing operator 
%\newcommand{\inducingoperator}[1][]{\ksdoperator}
\newcommand{\mmdoperator}{(\targetdist - \approxdist)}
\newcommand{\ksdoperator}{\approxdist \opsub{\targetdist}}
\newcommand{\mmd}[3]{\operatorname{MMD}_{#1}(#2, #3)}

\newcommand{\feat}{\Phi} % Feature function = A(x - m(Q))f(||x - y||)
\newcommand{\statfeat}{F}  % stationary part of feature function
\newcommand{\statfeatscalar}{f}  % stationary part of feature function
\newcommand{\multfeat}{A} % multiplicative part of feature function
\newcommand{\statkernel}{\Psi} % stationary part of base kernel 
\newcommand{\statkernelscalar}{\psi} % stationary part of base kernel 
\newcommand{\basekernel}{k}  % base kernel = A(x - m(Q))Psi(||x - y||)A(x - m(Q))

\newcommand{\FSD}{\ensuremath{\operatorname{\mathrm{\Phi}SD}}\xspace}
\newcommand{\FSDs}{{\FSD}s\xspace}
\newcommand{\RFSD}{\ensuremath{\operatorname{R\mathrm{\Phi}SD}}\xspace}
\newcommand{\RFSDs}{{\RFSD}s\xspace}
\newcommand{\KSD}{\ensuremath{\operatorname{KSD}}\xspace}
\newcommand{\GKSD}{\ensuremath{\operatorname{GKSD}}}
\newcommand{\FGKSD}{\ensuremath{\operatorname{fGKSD}}\xspace}
\newcommand{\MMD}{\ensuremath{\operatorname{MMD}}}
\newcommand{\FGMMD}{\ensuremath{\operatorname{fGMMD}}\xspace}
\newcommand{\GMMD}{\ensuremath{\operatorname{GMMD}}}
\newcommand{\IPM}{\ensuremath{\operatorname{IPM}}}
